LanguageMPC: Large Language Models as Decision Makers for Autonomous Driving

Existing learning-based autonomous driving (AD) systems face challenges in comprehending high-level information, generalizing to rare events, and providing interpretability. To address these problems, this work employs Large Language Models (LLMs) as a decision-making component for complex AD scenarios that require human commonsense understanding. We devise cognitive pathways to enable comprehensive reasoning with LLMs, and develop algorithms for translating LLM decisions into actionable driving commands. Through this approach, LLM decisions are seamlessly integrated with low-level controllers by guided parameter matrix adaptation. Extensive experiments demonstrate that our proposed method not only consistently surpasses baseline approaches in single-vehicle tasks, but also helps handle complex driving behaviors even multi-vehicle coordination, thanks to the commonsense reasoning capabilities of LLMs. This paper presents an initial step toward leveraging LLMs as effective decision-makers for intricate AD scenarios in terms of safety, efficiency, generalizability, and interoperability. We aspire for it to serve as inspiration for future research in this field. Project page: https://sites.google.com/view/llm-mpc

==> related_old.tex <==
\section{Related Work}

\noindent \textbf{Autonomous Driving Autonomy.}
Modularity~\cite{thrun2006stanley,daudelin2018integrated,chen2015deepdriving,8317797} plays an important role in many autonomous driving systems. It divides the complex autonomous driving task into multiple subproblems, including perception~\cite{li2023logonet,li2022bevformer,yin2021center}, planning~\cite{kelly2003reactive,zhang2022rethinking}, and control~\cite{peng2018sim,johnson2005pid}, making each module relevant and somewhat interpretable. However, it also presents challenges in areas such as compatibility, error accumulation and inefficiency\cite{chib2023recent}. 
Recently, there was a large progress in end-to-end deep learning methods for autonomous systems~\cite{casas2021mp3,uniad,sadat2020perceive,tampuu2020survey}. 
Though autonomous driving systems have achieved remarkable successes in planning and decision-making~\cite{kelly2003reactive,zhang2022rethinking,10160326}, there are still problems in terms of interpretability~\cite{gohel2021explainable,arrieta2019explainable,article,chib2023recent}. At the same time, limitations in data and sampling efficiency~\cite{atakishiyev2023explainable} make it vulnerable to dealing with long-tail situations, especially interaction scenarios, in real-world environments~\cite{kong2023robo3d}.

\noindent \textbf{Large Language Models for Autonomous Driving.}
The remarkable achievements of LLMs are undeniably captivating, demonstrating LLM's human-like reasoning skills and generalization of human commonsense~\cite{bian2023chatgpt,nay2022law,chowdhery2022palm,ouyang2022training,chung2022scaling}.
In the autonomous driving industry, LLMs have the potential to revolutionize the paradigm of perception and decision-making. On the perceptual side, researchers combine visual encoders with LLM~\cite{radford2021learning} to enhance the AD system's understanding of visual high-level concepts contained in images~\cite{liu2023visual} and videos~\cite{zhang2023videollama}. Recent works such as DriveGPT4~\cite{xu2024drivegpt4}, HiLM-D~\cite{ding2023hilmd}, and Talk2BEV~\cite{choudhary2023talk2bev} have even demonstrated the powerful environment perception capabilities of LLMs enabled by vectorized visual embedding techniques.
In planning and decision-making, extensive research has shown that pre-trained LLMs integrate human common sense and help make human-like decisions~\cite{huang2022language, huang2023voxposer, cui2023drive, wen2024dilu}.
Also, the involvement of LLMs greatly enhances interpretability and safety, providing the potential to comprehend the transparency of the decision process. \cite{xu2024drivegpt4, cui2023drive, 10611018} showed that LLMs can reason about the transportation environment under the guidance of prompt and explain the decision process. 
In addition, LLMs show the potential to address interoperability challenges~\cite{chen2023driving, kamath2023new}. \cite{mao2023gptdriver, jin2023surrealdriver, keysan2023text} uses language as a bridge between multimodal data, enabling the union of perception and decision-making, demonstrating powerful understanding and reasoning.
However, the above work mainly focuses on demonstrating the perception, reasoning and high-level decision-making capabilities of LLMs, which are still lacking in generating final control actions.
While \cite{fu2023drive, mao2023gptdriver} can generate planning trajectories, \cite{fu2023drive} relies on predefined fixed rules, and \cite{mao2023gptdriver} still requires the output of LLMs to be decoded into trajectories using a deep learning model, and the decoder still faces the problem of being limited by the training set.
In this work, we combine the LLM directly with the controller MPC and use the powerful reasoning and decision-making capabilities of the LLM to directly guide the generation of the final control actions, allowing the LLM to drive like a human.

% \vspace{-0.6cm}
% \vspace{-0.61cm}
